FODVid: Flow-guided Object Discovery in Videos

Segmentation of objects in a video is challenging due to the nuances such as motion blurring, parallax, occlusions, changes in illumination, etc. Instead of addressing these nuances separately, we focus on building a generalizable solution that avoids overfitting to the individual intricacies. Such a solution would also help us save enormous resources involved in human annotation of video corpora. To solve Video Object Segmentation (VOS) in an unsupervised setting, we propose a new pipeline (FODVid) based on the idea of guiding segmentation outputs using flow-guided graph-cut and temporal consistency. Basically, we design a segmentation model incorporating intra-frame appearance and flow similarities, and inter-frame temporal continuation of the objects under consideration. We perform an extensive experimental analysis of our straightforward methodology on the standard DAVIS16 video benchmark. Though simple, our approach produces results comparable (within a range of ~2 mIoU) to the existing top approaches in unsupervised VOS. The simplicity and effectiveness of our technique opens up new avenues for research in the video domain.

==> 02related_work.tex <==
\section{Related Work}
\label{sec:relatedwork}

\textbf{Unsupervised Video Object Segmentation.}  The goal of video object segmentation (VOS) is to localize object(s) in a given video sequence. In the literature~\cite{li2013video, ochs2013segmentation, perazzi2016benchmark}, this problem is generally re-framed as foreground-background separation, where the most salient object in the video \textit{typically} forms the foreground. Prior works tackle this problem either in the semi-supervised~\cite{caelles2017one, hu2018unsupervised, lai2020mast} or unsupervised setup~\cite{tokmakov2017learning, choudhury2022guess, faktor2014video, li2018instance, lu2019see, papazoglou2013fast, tokmakov2019learning}. The inference setting of semi-supervised VOS requires the segmentation to be provided for the first frame and the goal is to accurately propagate them throughout the video. Recent works in the semi-supervised setting~\cite{xu2021rethinking, araslanov2021dense, lai2019self} follow the idea of learning good feature representations that can be used to find temporal correspondences in videos, thus producing semantic labels for all the frames. On the other hand, in the unsupervised setup, the annotations are not required even for the first frame. Despite not requiring any annotation during training, the unsupervised VOS methods still rely on \textit{supervised} pre-training on external data or optical flow models trained on annotated datasets. In contrast, to avoid any such leaky supervision, we propose a \textit{fully} unsupervised pipeline for the VOS task and achieve state-of-the-art results.  


\vskip 0.2cm
\textbf{Motion Segmentation.}  Optical flow provides rich visual cues for segmenting objects in a video, as a result of which many works have modelled the problem of unsupervised VOS as a motion segmentation problem~\cite{sundaram2010dense, keuper2017higher, keuper2015motion, keuper2018motion, tokmakov2017learning, yang2021dystab}. Models based on layer extraction~\cite{xie2022segmenting, ye2022deformable, chang2013topology, jojic2001learning}
decompose the video into layers of persistent motion groups, however leading to complex inference procedure. Brox \etal~\cite{brox2010object} use long term point trajectories derived from optical flow and cluster them based on pair-wise distances to get a temporally consistent segmentation of an object.~\cite{faktor2014video} cast the video segmentation problem as a voting scheme on the graph of co-occurring regions in the video sequence.~\cite{papazoglou2013fast} partition all the frames in a video into super-pixels and label each as foreground or background, encouraging foreground label for super-pixels that undergo independent motion.~\cite{yang2019unsupervised} propose to utilise an adversarial framework, wherein an inpainter network tries to predict optical flow in a region based on context, while another network makes that region as uninformative as possible. FusionSeg~\cite{dutt2017fusionseg} proposes to combine the appearance and motion modalities for segmentation. MG~\cite{yang2021self}, on the other hand, discards the appearance modality altogether, and instead segments motion itself via slot attention mechanism. AMD~\cite{liu2021emergence} uses two visual pathways to predict coherent object regions in RGB images and optical flow vectors for those regions. Another line of work involves modelling optical flow as a piecewise set of parametric motion models, typically affine or quadratic motion models~\cite{choudhury2022guess, meunier2022driven, jepson1993mixture, torr1998geometric, mahendran2018self}. On the contrary, we use optical flow RGB to distill \textit{rough} object masks from DINO, and further use it as a guidance to regularise the refinement process.


% \vskip 0.2cm
% \textbf{Unsupervised Object Discovery.}


\vskip 0.2cm
\textbf{Unsupervised Semantic Segmentation.}  We have considered the problem of VOS, which is binary segmentation of its frames into foreground (salient object(s)) and background regions. Earlier works relied on hand-crafted priors~\cite{cheng2014global, wei2012geodesic}, though they do not perform as well as deep learning methods~\cite{nguyen2019deepusps, zeng2019multi, zhang2018deep, ji2019invariant, ouali2020autoregressive, voynov2021object, melas2021finding, chen2019unsupervised, kanezaki2018unsupervised, benny2020onegan, bielski2019emergence}. \textbf{Should we write these?..} For completeness sake, we briefly outline works in dense unsupervised semantic segmentation as well. The goal of dense semantic segmentation is to assign a class label for every pixel in an image. Recent works~\cite{hamilton2022unsupervised, Melas-Kyriazi_2022_CVPR, chen2022unsupervised, ziegler2022self, wang2022self, henaff2022object, ke2022unsupervised, van2021unsupervised, cho2021picie} learn discriminative representations of patches or pixels in an image, which can be clustered in the feature space to produce a semantic segmentation. Our model architecture is designed in such a way that the model is trained on videos but still takes a \textit{single} image as input for segmentation.


